Enhancing Steering Estimation with Semantic-Aware GNNs

Steering estimation is a critical task in autonomous driving, traditionally relying on 2D image-based models. In this work, we explore the advantages of incorporating 3D spatial information through hybrid architectures that combine 3D neural network models with recurrent neural networks (RNNs) for temporal modeling, using LiDAR-based point clouds as input. We systematically evaluate four hybrid 3D models, all of which outperform the 2D-only baseline, with the Graph Neural Network (GNN) - RNN model yielding the best results. To reduce reliance on LiDAR, we leverage a pretrained unified model to estimate depth from monocular images, reconstructing pseudo-3D point clouds. We then adapt the GNN-RNN model, originally designed for LiDAR-based point clouds, to work with these pseudo-3D representations, achieving comparable or even superior performance compared to the LiDAR-based model. Additionally, the unified model provides semantic labels for each point, enabling a more structured scene representation. To further optimize graph construction, we introduce an efficient connectivity strategy where connections are predominantly formed between points of the same semantic class, with only 20\% of inter-class connections retained. This targeted approach reduces graph complexity and computational cost while preserving critical spatial relationships. Finally, we validate our approach on the KITTI dataset, achieving a 71% improvement over 2D-only models. Our findings highlight the advantages of 3D spatial information and efficient graph construction for steering estimation, while maintaining the cost-effectiveness of monocular images and avoiding the expense of LiDAR-based systems.

==> sections/related_works_.tex <==
\section{Related works}



Graph convolutional networks (GCNs) have gained significant traction for processing structured data, including applications in image and document classification, as well as semi-supervised learning.







"3D Point Cloud Processing and Learning for
Autonomous Driving"

We present a review of 3D point cloud processing
and learning for autonomous driving.



"Pointnet"

The motivation of using
PointNet-based methods is to directly handle raw 3D points
by deep neural networks without any discretization. PointNet [7] is a pioneering work that achieves this goal. Raw
3D point clouds are inherently unordered sets, and PointNet
was designed to respect this property and produce the same
output regardless of the ordering of the input data. The key
technical contribution of PointNet is to use a set of shared
point-wise multi-layer perceptrons (MLPs) followed by global
pooling to extract geometric features while ensuring this
permutation-invariant property of raw 3D data. Even though
the architecture is simple, it has become a standard building
block for numerous 3D point cloud learning algorithms and
achieves surprisingly strong performance on 3D point cloud
recognition and segmentation.

since each 3D point
goes through the same MLPs separately and the max-pooling
removes the point dimension, the entire computational block
is permutation invariant; that is, the ordering of 3D points
does not influence the output of this block



------------

Graph-based methods. The motivation of using graphbased methods is to leverage the spatial relationships among
3D points to accelerate the end-to-end learning of deep neural
networks

 To capture the local relationships
among 3D points, one can introduce a graph structure, where
each node is a 3D point and each edge reflects the relationship
between each pair of 3D points. This graph structure is a
discrete proxy of the surface of an original object


There are several ways to construct a graph, such as a
K-nearest-neighbor graph, an -graph and a learnable graph.
A K-nearest-neighbor graph is a graph in which two nodes
are connected by an edge, when their Euclidean distance is
among the K-th smallest Euclidean distances from one 3D
point to all the other 3D points. An -nearest-neighbor graph
is a graph in which two nodes are connected by an edge,
when their Euclidean distance is smaller than a given threshold . Both K-nearest-neighbor graphs and -graphs can be
efficiently implemented by using efficient data structures, such
as Octree [11]. A learnable graph is a graph whose adjacency
matrix is trainable in an end-to-end learning architecture.


----------------------------------

3D Graph Neural Networks for RGBD Semantic Segmentation

In
this paper we propose a 3D graph neural network (3DGNN)
that builds a k-nearest neighbor graph on top of 3D point
cloud. Each node in the graph corresponds to a set of points
and is associated with a hidden representation vector initialized with an appearance feature extracted by a unary
CNN from 2D images. Relying on recurrent functions, every
node dynamically updates its hidden representation based
on the current status and incoming messages from its neighbors. This propagation model is unrolled for a certain number of time steps and the final per-node representation is
used for predicting the semantic class of each pixel.


Several methods [11, 29, 21, 7] treat RGBD segmentation as a 2D segmentation problem where depth is taken as
another input image. Deep convolutional neural networks
(CNNs) are applied separately to the color and depth images to extract features. (do not forget to talk about your arxiv paper where one cnn is used)



An alternative is to use 3D CNNs [37] in voxelized
3D space. This type of methods has the potential to extract more geometric information. However, since 3D point
clouds are quite sparse, effective representation learning
from such data is challenging. In addition, 3D CNNs are
computationally more expensive than their 2D version, thus
it is difficult to scale up these systems to deal with a large
number of classes


We first cast the 2D pixels into 3D based on depth information and associate with each 3D
point a unary feature vector, i.e., an output of a 2D segmentation CNN. We then build a graph whose nodes are these
3D points, and edges are constructed by finding the nearest
neighbors in 3D. For each node, we take the image feature
vector as the initial representation and iteratively update it
using a recurrent function. The key idea of this dynamic
computation scheme is that the node state is determined
by its history state and the messages sent by its neighbors,
while taking both appearance and 3D information into consideration

scuss their relationship with existing models.
For GNNs, the input data is represented as a graph G =
{V, E}, where V and E are the sets of nodes and edges of
the graph, respectively


A Graph Neural Network is a dynamic model where the
hidden representation of all nodes evolve over time. At time
step t, the hidden representation is updated as
mt
v = M

{h
t
% u|u ∈ Ωv}
% 
% h
% t+1
% v = F

% h
% t
% , mt
% v
% 
, (1)
where mt
v
is a vector, which indicates the aggregation of
messages that node v receives from its neighbors Ωv. M is
a function to compute the message and F is the function to
update the hidden state. Similar to a recurrent neural network, M and F are feedforward neural networks that are
shared among different time ste

. Graph Construction
Given an image, we construct a directed graph based on
the 2D position and the depth information of pixels. 

To form our graph, we regard each pixel as a node and connect it via directed edges to K nearest neighbors (KNN) in
the 3D space, where K is set to 64 in our experiments. Note
that this process creates asymmetric structure, i.e., an edge
from A to B does not necessarily imply existence of the
edge from B to A


After constructing the graph, we use a CNN as the unary
model to compute the features for each pixel. Taking these features as the initial hidden representation of the corresponding node, we encode
the appearance information. Given that the 3D graph already encodes the geometric context, this graph neural network exploits both appearance and geometry information. s. The
message is computed by first feeding hidden states to the
MLP g and then taking the average over the neighborhood.
Then every node updates its hidden state based on previous
state and the aggregated message. 


-------------------------------------

Spatial Temporal Graph Convolutional Networks for Skeleton-Based Action
Recognition

Graph Neural networks (GCNs), which generalize
convolutional neural networks (CNNs) to graphs of arbitrary
structures, have received increasing attention and successfully
been adopted in a number of applications, such as
image classification (Bruna et al. 2014), document classification
(Defferrard, Bresson, and Vandergheynst 2016), and
semi-supervised learning (Kipf and Welling 2017).

In this paper, we propose to design a generic representation
of skeleton sequences for action recognition by extending
graph neural networks to a spatial-temporal graph
model, called Spatial-Temporal Graph Convolutional Networks
(ST-GCN).


There
are two types of edges, namely the spatial edges that conform
to the natural connectivity of joints and the temporal
edges that connect the same joints across consecutive time
steps. Multiple layers of spatial temporal graph convolution
are constructed thereon, which allow information to be integrated
along both the spatial and the temporal dimension.


The major contributions of this work lie in three aspects:
1) We propose ST-GCN, a generic graph-based formulation
for modeling dynamic skeletons, which is the first that applies
graph-based neural networks for this task. 2) We propose
several principles in designing convolution kernels in
ST-GCN to meet the specific demands in skeleton modeling.

he discussed neural network
architectures include both recurrent neural networks (Tai,
Socher, and Manning 2015; Van Oord, Kalchbrenner, and
Kavukcuoglu 2016) and convolutional neural networks
(CNNs) (Bruna et al. 2014; Henaff, Bruna, and LeCun 2015;
Duvenaud et al. 2015; Li et al. 2016; Defferrard, Bresson,
and Vandergheynst 2016). This work is more related to the
generalization of CNNs, or graph convolutional networks
(GCNs). The principle of constructing GCNs on graph generally
follows two streams: 1) the spectral perspective,
where the locality of the graph convolution is considered
in the form of spectral analysis (Henaff, Bruna, and Le-
Cun 2015; Duvenaud et al. 2015; Li et al. 2016; Kipf and
Welling 2017); 2) the spatial perspective, where the convolution
filters are applied directly on the graph nodes and their
neighbors (Bruna et al. 2014; Niepert, Ahmed, and Kutzkov
2016). This work follows the spirit of the second stream. 

We construct the CNN filters on the spatial domain, by limiting
the application of each filter to the 1-neighbor of each node. 


We construct the spatial temporal
graph on the skeleton sequences in two steps. First, the
joints within one frame are connected with edges according
to the connectivity of human body structure, which is
illustrated in Fig. 1. Then each joint will be connected to
the same joint in the consecutive frame.


----------------------------

Social-STGCNN: A Social Spatio-Temporal Graph Convolutional Neural
Network for Human Trajectory Prediction

Pedestrian
trajectories are not only influenced by the pedestrian itself
but also by interaction with surrounding objects. 

We propose the Social Spatio-Temporal Graph
Convolutional Neural Network (Social-STGCNN), which
substitutes the need of aggregation methods by modeling the
interactions as a graph


Graph CNNs were
introduced by [8] which extends the concept of CNNs into
graphs. The Convolution operation defined over graphs is
a weighted aggregation of target node attributes with the
attributes of its neighbor nodes. It is similar to CNNs but the
convolution operation is taken over the adjacency matrix of
the graphs. The works [9, 4, 24] extend the graph CNNs to
other applications such as matrix completion and Variational
Auto Encoders.

 The ST-GCNN conducts spatiotemporal convolution operations on the graph representation
of pedestrian trajectories to extract features. These features are a compact representation of the observed pedestrian trajectory history. TXP-CNN takes these features as inputs and
predicts the future trajectories of all pedestrians as a whole.

s We
first introduce the construction of the graph representation
of pedestrian trajectories. We start by constructing a set
of spatial graphs Gt representing the relative locations of
pedestrians in a scene at each time step t. 



TPCN: Temporal Point Cloud Networks for Motion Forecasting


s. Instead of directly
applying works [26, 27, 33, 36] whose computation cost is
high, we propose our novel spatial learning layer, namely
Dual-representation Spatial Learning to obtain pointwise
and voxelwise features through point cloud learning. Meanwhile, we propose Dynamic Temporal Learning in the
temporal module to effectively extract the time-series information and motion estimation


GCN based methods. Graph Convolutional Network
(GCN) [8, 13, 30] nowadays gains its popularity in processing non-structural data and dealing with correlation relationship. Compared with traditional CNN, GCN shows its
great promise in capturing the spatial locality on both euclidean and non-euclidean structures. With adjacency matrices, GCN focuses on learning the relationship between
graph nodes and vertices. VectorNet [10] introduces a novel
vector representation and applies a graph neural network to
predict the intent of vehicles. M Liang et al. [19] proposes
LaneGCN based on GCN, which is a specialized version
designed for lane graphs. In order to capture the complex
topology of HD maps effectively, it combines with multiscale dilated convolution. Social-STGCNN [24] models interactions as a graph by defining a novel kernel function to
learn spatial and temporal patterns from pedestrian trajectories and behavior. However, GCN based methods are often
faced with an efficiency problem when dealing with largescale scenarios that contain lots of nodes and vertices.


GCN based methods. Graph Convolutional Network
(GCN) [8, 13, 30] nowadays gains its popularity in processing non-structural data and dealing with correlation relationship. Compared with traditional CNN, GCN shows its
great promise in capturing the spatial locality on both euclidean and non-euclidean structures. With adjacency matrices, GCN focuses on learning the relationship between
graph nodes and vertices. VectorNet [10] introduces a novel
vector representation and applies a graph neural network to
predict the intent of vehicles. M Liang et al. [19] proposes
LaneGCN based on GCN, which is a specialized version
designed for lane graphs. In order to capture the complex
topology of HD maps effectively, it combines with multiscale dilated convolution. Social-STGCNN [24] models interactions as a graph by defining a novel kernel function to
learn spatial and temporal patterns from pedestrian trajectories and behavior. However, GCN based methods are often
faced with an efficiency problem when dealing with largescale scenarios that contain lots of nodes and vertices

The overall network architecture of our TPCN approach
consists of two modules: 1) Dual-representation Spatial
Learning and 2) Dynamic Temporal Learning. The Dualrepresentation Spatial Learning serves as the spatial module to model spatial features, and the Dynamic Temporal
Learning is the temporal module to extract temporal features. Both modules are integrated to propagate features
mutually in spatial and temporal dimensions to achieve
Joint Learning. As shown in Fig. 1, each module takes the
pointwise features of the other module as input to generate
corresponding pointwise output features, which is a natural
foundation for fusing pointwise context information across
multiple domains:
    Pointwise Feature Learning. Pointwise features maintain geometric information and neighborhood relationship
for interactions among points. To this end, we utilize the hierarchical feature learning from PointNet++ [27] for pointwise feature extraction at different levels of the local neighborhood to exploit more local structure and correlation

    Dual-representation Fusion. With pointwise and voxelwise features, we fuse these two types of features by feature concatenation. Thus, we obtain the features with dual
representations and higher context information, which will
be passed to the next stage of dynamic temporal learning








PointNet++: Deep Hierarchical Feature Learning on
Point Sets in a Metric Space

PointNet [20] is a pioneering effort that directly
processes point sets. The basic idea of PointNet is to learn a spatial encoding of each point and then
aggregate all individual point features to a global point cloud signature. By its design, PointNet does
not capture local structure induced by the metric. However, exploiting local structure has proven to
be important for the success of convolutional architectures. A CNN takes data defined on regular
grids as the input and is able to progressively capture features at increasingly larger scales along a
multi-resolution hierarchy. At lower levels neurons have smaller receptive fields whereas at higher
levels they have larger receptive fields. The ability to abstract local patterns along the hierarchy
allows better generalizability to unseen cases
    


We introduce a hierarchical neural network, named as PointNet++, to process a set of points sampled
in a metric space in a hierarchical fashion. The general idea of PointNet++ is simple. We first
partition the set of points into overlapping local regions by the distance metric of the underlying
space. Similar to CNNs, we extract local features capturing fine geometric structures from small
neighborhoods; such local features are further grouped into larger units and processed to produce
higher level features. This process is repeated until we obtain the features of the whole point set.



 PointNet++ applies PointNet
recursively on a nested partitioning of the input set.


 To
evenly cover the whole set, the centroids are selected among input point set by a farthest point
sampling (FPS) algorithm. Compared with volumetric CNNs that scan the space with fixed
strides, our local receptive fields are dependent
on both the input data and the metric, and thus
more efficient and effective. 


A significant contribution of our paper is that PointNet++ leverages neighborhoods at multiple scales
to achieve both robustness and detail capture. Assisted with random input dropout during training,
the network learns to adaptively weight patterns detected at different scales and combine multi-scale
features according to the input data.


Our work can be viewed as an extension of PointNet [20] with added hierarchical structure

Our hierarchical structure is composed by a number of set abstraction levels (Fig. 2). At each level, a
set of points is processed and abstracted to produce a new set with fewer elements. The set abstraction
level is made of three key layers: Sampling layer, Grouping layer and PointNet layer. The Sampling
layer selects a set of points from input points, which defines the centroids of local regions. Grouping
layer then constructs local region sets by finding “neighboring” points around the centroids. PointNet
layer uses a mini-PointNet to encode local region patterns into feature vectors.



each abstraction level contains grouping and feature extraction of a single scale.
In PointNet++, each abstraction level extracts multiple scales of local patterns and combine them
intelligently according to local point densities. In terms of grouping local regions and combining
features from different scales, we propose two types of density adaptive layers as listed below



each abstraction level contains grouping and feature extraction of a single scale.
In PointNet++, each abstraction level extracts multiple scales of local patterns and combine them
intelligently according to local point densities. In terms of grouping local regions and combining
features from different scales, we propose two types of density adaptive layers as listed below (MSG and MRG)





3D Recurrent Neural Networks with Context
Fusion for Point Cloud Semantic Segmentation


In this paper, a novel end-to-end approach
for unstructured point cloud semantic segmentation, named 3P-RNN,
is proposed to exploit the inherent contextual features. First the efficient pointwise pyramid pooling module is investigated to capture local
structures at various densities by taking multi-scale neighborhood into
account. Then the two-direction hierarchical recurrent neural networks
(RNNs) are utilized to explore long-range spatial dependencies. Each recurrent layer takes as input the local features derived from unrolled cells
and sweeps the 3D space along two directions successively to integrate
structure knowledge.


Voxel-based 3D CNNs: In order to represent 3D geometric shape, a point
cloud is first converted into regular volumetric occupancy grids and then trained
by 3D CNNs to yield voxel-level predictions [7, 11, 12]. However, uniform 3D
arrangement is inefficient because of the sparsity of 3D data. Besides, due to
the expensive computation of 3D convolutions than 2d ones, the voxel size is
constrained to a relatively small size and accordingly, it is challenging for such
architectures to be extended to large-scale point clouds. Unbalanced octrees were
exploited to tackle the sparsity problem, which allowed to train 3D CNNs at
higher resolutions [13]. SEGCloud subsampled large cloud into voxels and postprocessed by trilinear interpolation and conditional random field [14]. However,
all the voxel-based methods fail to achieve point-level accuracy


Deep learning on unordered point sets: PointNet [4] was the first architecture that directly worked on raw point sets to produce per-point classes.
Pointwise features and the aggregated global feature were concatenated to make pointwise predictions. However, the absence of neighboring context structure
limited the segmentation performance on complicated scenes. To overcome this
drawback, the hierarchical approach PointNet++ [22] was designed to better capture local structures as well as generalize to variable densities. Also inspired by
the recent PointNet work, multi-scale windows or neighboring cell positions were
exploited to incorporate neighborhood knowledge [23]. Due to the efficiency in
extracting point-features, the PointNet framework was further extended to learn
local shape properties [24] as well as predict 3D Object Detection from RGB-D
Data [25]. Graph neural networks (GNNs) were undertaken to spread contextual
information on top of 3D points [26]. Nevertheless, each node in the k-nearest
neighbor graph requires additional 2D appearance features for initialization. A
very recent GNN work captured the structure of point clouds by superpoint
graph, which partitioned various objects into simple shapes and assigned segmentation labels to each part as a whole [27]. The GNNs iteratively updated the
node state by message propagation over neighboring nodes. 


The proposed framework takes inspiration from PointNet [4], which is briefly
reviewed in the following part. The baseline is extended with two distinctive
improvements to learn local and long-dependency spatial context for better performance. For one thing, a pointwise pyramid pooling module is proposed to
learn multi-scale neighboring context. Though simple, it is more efficient than
multi-scale input context aggregation in [22, 23] because of the non-parametric
pooling units. For another, long-range context is exploited by the two-direction
RNN model, which enables the network to learn spatial context in large-scale
point clouds.



End-to-End Neural Network for Autonomous
Steering using LiDAR Point Cloud Data


This study investigates a LiDAR point cloud-based endto-end autonomous steering problem in structured roads. The
control command to the vehicle is focused on the steering angle
of the wheel, which is discretized into continuous integers as
the direction category. The problem is then converted into a
classification task, which is a mapping connection between the
original point cloud data and the driving direction category. On
the basis of the PointNet++ framework, we propose using Kmeans, KNN, and weighted sampling, to perform the steering
decision making. Using the CARLA simulation environment, we
have shown that the proposed approach is performing effective
autonomous decision making with a rate strictly higher than 91%
while requiring less inference speed compared to benchmarks.



In order to facilitate the experiment, we linearly discretize
the steering wheel angle into an integer between [0, 180], and
convert it into a classification problem


PointNet can only perform the MaxPooling operation after
extracting single-point features, and does not extract local
features. Therefore, the primitive PointNet model has a weak
ability to describe the point cloud features in the local neighborhood, which makes the local features learned in the process
of training and testing insufficient
    thats why we use pointnet++ instead






VectorNet: Encoding HD Maps and Agent Dynamics from
Vectorized Representation


 This paper introduces VectorNet, a hierarchical
graph neural network that first exploits the spatial locality
of individual road components represented by vectors and
then models the high-order interactions among all components


The core
interest is to find a unified representation which integrates
the agent dynamics, acquired by perception systems such as object detection and tracking, with the scene context, provided as prior knowledge often in the form of High Definition (HD) maps. Our goal is to build a system which learns
to predict the intent of vehicles, which are parameterized as
trajectories

We propose to learn a unified representation for multiagent dynamics and structured scene context directly from
their vectorized form.  The geographic extent of the road features can be a point, a polygon, or a curve
in geographic coordinates. All these
polylines can then be represented as sets of vectors


We use graph neural networks (GNNs) to incorporate
these sets of vectors. We treat each vector as a node in
the graph, and set the node features to be the start location
and end location of each vector, along with other attributes
such as polyline group id and semantic labels. The context
information from HD maps, along with the trajectories of
other moving agents are propagated to the target agent node
through the GNN. We can then take the output node feature corresponding to the target agent to decode its future
trajectories.

Specifically, to learn competitive representations with
GNNs, we observe that it is important to constrain the connectivities of the graph based on the spatial and semantic
proximity of the nodes. We therefore propose a hierarchical graph architecture, where the vectors belonging to the
same polylines with the same semantic labels are connected
and embedded into polyline features, and all polylines are
then fully connected with each other to exchange information. We implement the local graphs with multi-layer perceptrons, and the global graphs with self-attention
    similarly, but in our case we keep 20\% connected even if they are not belonging to the same semantics
